Unlocking Profit Potential: Maximizing Returns with Bayesian Optimization of Supertrend Indicator Parameters

This paper investigates the potential of Bayesian optimization (BO) to optimize the atr multiplier and atr period -the parameters of the Supertrend indicator for maximizing trading profits across diverse stock datasets. By employing BO, the thesis aims to automate the identification of optimal parameter settings, leading to a more data-driven and potentially more profitable trading strategy compared to relying on manually chosen parameters. The effectiveness of the BO-optimized Supertrend strategy will be evaluated through backtesting on a variety of stock datasets.

==> title.tex <==

%----------------------------------------------------------------------------------------
%	TITLE SECTION
%----------------------------------------------------------------------------------------

\HRule \\[0.4cm]
{ \huge \bfseries Report}\\ % Title of your document
\HRule \\[1.5cm]
\end{center}
%----------------------------------------------------------------------------------------
%	AUTHOR SECTION
%----------------------------------------------------------------------------------------

%\begin{minipage}{0.4\hsize}
\begin{flushleft} \large
\textit{Abdul Rahman}\\
% \reportauthorOne~(ID: \cidOne)\\ % Your name
% \reportauthorTwo~(ID: \cidTwo)
MA22C001% Your name
\end{flushleft}
\begin{flushright}\large
\textit{\underline{Advisor} }\\
% \reportauthorOne~(ID: \cidOne)\\ % Your name
% \reportauthorTwo~(ID: \cidTwo)
Dr.Neelesh Upadhye\\
IIT Madras% Your name
\end{flushright}
\vspace{4cm}
\makeatletter
Date: \@date 

\vfill % Fill the rest of the page with whitespace



\makeatother


\end{titlepage}
